CT-Wasm: Type-Driven Secure Cryptography for the Web Ecosystem

A significant amount of both client and server-side cryptography is implemented in JavaScript. Despite widespread concerns about its security, no other language has been able to match the convenience that comes from its ubiquitous support on the "web ecosystem" - the wide variety of technologies that collectively underpins the modern World Wide Web. With the new introduction of the WebAssembly bytecode language (Wasm) into the web ecosystem, we have a unique opportunity to advance a principled alternative to existing JavaScript cryptography use cases which does not compromise this convenience. We present Constant-Time WebAssembly (CT-Wasm), a type-driven strict extension to WebAssembly which facilitates the verifiably secure implementation of cryptographic algorithms. CT-Wasm's type system ensures that code written in CT-Wasm is both information flow secure and resistant to timing side channel attacks; like base Wasm, these guarantees are verifiable in linear time. Building on an existing Wasm mechanization, we mechanize the full CT-Wasm specification, prove soundness of the extended type system, implement a verified type checker, and give several proofs of the language's security properties. We provide two implementations of CT-Wasm: an OCaml reference interpreter and a native implementation for Node.js and Chromium that extends Google's V8 engine. We also implement a CT-Wasm to Wasm rewrite tool that allows developers to reap the benefits of CT-Wasm's type system today, while developing cryptographic algorithms for base Wasm environments. We evaluate the language, our implementations, and supporting tools by porting several cryptographic primitives - Salsa20, SHA-256, and TEA - and the full TweetNaCl library. We find that CT-Wasm is fast, expressive, and generates code that we experimentally measure to be constant-time.

==> GNUmakefile <==
MAIN = paper.tex
PDF = pdf

ifeq ($(PDF),pdf)
FIGEXT    = pdf
OUTEXT    = pdf
else
FIGEXT    = eps
OUTEXT    = dvi
endif

BASE      := $(basename $(MAIN))
SRCEXT    := $(patsubst $(BASE).%,%,$(MAIN))
XFIGS     := $(wildcard *.fig)
DIAFIGS   := $(wildcard *.dia)
SVGFIGS   := $(wildcard *.svg)
TEXFIGS   := $(XFIGS:.fig=.tex) # $(DIAFIGS:.dia=.tex)
BINFIGS   := $(XFIGS:.fig=.$(FIGEXT)) $(DIAFIGS:.dia=.$(FIGEXT)) $(SVGFIGS:.svg=.$(FIGEXT)) $(GENFIGS)
STYLINK	  := $(notdir $(wildcard ../*.sty))
STYFILES  := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES  := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES) $(TEXFIGS))
BIBFILES  := $(wildcard *.bib)
EPLOTS	  := $(wildcard eval/*.gnuplot)
JGRAPHS   := $(wildcard *.j)
GGRAPHS   := $(wildcard *.gnuplot)
GRAPHS    := $(JGRAPHS.j=.$(FIGEXT)) $(GGRAPHS:.gnuplot=.$(FIGEXT))

ifeq ($(PDF),pdf)
IMAGESRC  := $(wildcard figs/*.gif) $(wildcard figs/*.eps) 
else
IMAGESRC  := $(wildcard figs/*.gif) 
endif
IMAGEGEN  := $(addsuffix .$(FIGEXT), $(basename $(IMAGESRC)))
IMAGES    := $(sort $(IMAGEGEN) $(wildcard figs/*.$(FIGEXT)))
IMAGEDIST := $(filter-out $(IMAGEGEN), $(IMAGES)) \
		$(wildcard figs/*.odp) $(wildcard figs/*.ppt)

ifeq ($(PDF),pdf)
LATEX     = pdflatex -synctex=1 -shell-escape -halt-on-error -interaction=nonstopmode
#\nonstopmode\\input
else
LATEX     = latex
#\\nonstopmode\\input
DVIPS     = dvips -j0 -G0 -t letter -Pdownload35
PS2PDF    = GS_OPTIONS=-sPAPERSIZE=letter ps2pdf -sPAPERSIZE=letter -dEmbedAllFonts=true
#PS2PDF    = ps2pdf
endif
BIBTEX    = bibtex -min-crossrefs=1000

all: $(BASE).pdf

crop: $(BASE).pdf
	pdfcrop --margins 15 $(BASE).pdf

ifeq ($(PDF),pdf)
%.pdf %.tex: %.fig
	fig2dev -L pdftex -p1 $< > $*.pdf
	fig2dev -L pdftex_t -p $*.pdf $< > $*.tex

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

figs/%.pdf: figs/%.gif
	convert $< $@

%.ps: %.pdf
	pdftops -paper A4 $< $@

else
%.ps: %.dvi
	$(DVIPS) $< -o $@

%.eps %.tex: %.fig
	fig2dev -L pstex -p1 $< > $*.eps
	fig2dev -L pstex_t -p $*.eps $< > $*.tex
endif

%.eps: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.tex: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.eps: %.j
	@rm -f $@~
	jgraph $< > $@~
	mv -f $@~ $@
%.eps: %.gnuplot %.data
	gnuplot $*.gnuplot
%.pdf: %.svg
	inkscape -z -A $@ $< && cp $@ .missing/$@ || cp .missing/$@ $@

$(STYLINK):
	rm -f $@
	ln -s ../$@ .

RERUN = egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' $*.log
UNDEFINED = egrep -q '^(LaTeX|Package natbib) Warning:.* undefined' $*.log

# So you can "setenv ALWAYS yes" instead of butchering the Makefile...
ifneq ($(ALWAYS),)
ALWAYS = always
endif
$(BASE).$(OUTEXT): %.$(OUTEXT): %.$(SRCEXT) $(TEXFILES) $(BIBFILES) \
				$(BINFIGS) $(GRAPHS) $(IMAGES) $(ALWAYS)
	test ! -s $*.aux || $(BIBTEX) $* || rm -f $*.aux $*.bbl
	$(LATEX) $< || ! rm -f $@
	if $(UNDEFINED); then \
		$(BIBTEX) $* && $(LATEX) $< || ! rm -f $*.bbl $@; \
	fi
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
ifeq ($(PDF),pdf)
	touch $*.dvi
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
else
$(BASE).pdf: %.pdf: %.ps
	$(PS2PDF) $< $@
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
endif

DIST = GNUmakefile $(filter-out $(TEXFIGS), $(TEXFILES)) \
	$(XFIGS) $(DIAFIGS) $(SVGFIGS) $(GENFIGSRC) \
	$(JGRAPHS) $(GGRAPHS) $(GGRAPHS:.gnuplot=:.data) \
	$(IMAGESRC) $(IMAGEDIST) $(BIBFILES)
dist: $(BASE).tar.gz
$(BASE).tar.gz: $(DIST)
	tar -chzf $@ -C .. \
		$(patsubst %, $(notdir $(PWD))/%, $(DIST))

PREVIEW := $(BASE)
preview: $(PREVIEW).pdf
	if test -f .xpdf-running; then			\
		xpdf -remote $(BASE)-server -quit;	\
		sleep 1;				\
	fi
	touch .xpdf-running
	(xpdf -remote $(BASE)-server $(PREVIEW).pdf; rm -f .xpdf-running) &

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

check:
	pdflatex $(BASE).ltx | grep -e "multiply" -e "undefined"

EXTRAIGNORE = '*~' '*.aux' '*.bbl' '*.blg' '*.log' '*.dvi' '*.bak' '*.out'
ignore:
	rm -f .gitignore
	(for file in $(EXTRAIGNORE); do \
		echo "$$file"; \
	done; \
	for file in .xpdf-running \
			$(BASE).tar.gz \
			$(TEXFIGS) $(BINFIGS) $(GRAPHS) $(IMAGEGEN) \
			$(BASE).ps $(BASE).pdf; do \
		echo "/$$file"; \
	done) | sort > .gitignore
	git add .gitignore

clean:
	rm -f $(BASE).ps $(BASE).pdf $(BASE).tar.gz
	rm -f $(TEXFIGS) $(GRAPHS) # $(IMAGEGEN)
	rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out
	rm -f *~ *.core core

binfigsclean: clean
	rm -f $(BINFIGS)

always:
	@:

.PHONY: install clean binfigsclean all always ignore preview show osx dist

spell:
	make clean
	for i in $(wildcard *.tex); do aspell -p ./aspell.words -c $$i; done

flat:
	./flatten.pl $(MAIN) > $(BASE)-flat.tex

proof:
	./weasel *.tex
	./passive *.tex


==> TODOS <==
# Small todos
- [ ] Fig 1 make not shit + caption should explain wtf this is
- [ ] Section vs. \S
- [ ] behavior vs. behaviour and other english things
- [x] Use Fig vs. Figure
- [x] move public memory imports to supplemental. inline the results when we talk bout multiple memories
- [x] Move table on pg 24 to supplemntal.
- [x] TweetNacl mention number of functions and LOC
- [x] Fig 7 will be fixed by deian
- [ ] Vanilla instead of unmodified
- [x] Fig 8 key is fucked up. Fix caption too
- [x] Fig 8 put TEA and john will explain; explain what size messages; add y axis
- [x] Fig 9 + 10, subfig side by side, bold 10
- [ ] deian add citation to node drama
- [ ] don't use label when we use annotations everywhere else
- [ ] K and KK usage consitancy
- [ ] use K insteadof texttt
- [x] Natalies public memory benchmark should be in supplemental


==> figures/fig-syntax__copy_.tex <==
%!TEX root = ../paper.tex

\begin{figure*}
$$
\fontsize{8pt}{8pt}
\begin{array}{@{}ll@{}}
\begin{array}[b]{@{}llcl@{}}
\text{(values)} & \x{v} &::=&
  t\KK{.const}~c \\
\text{(store index)} & \x{a} &::=&
  \x{i} \\
\text{(module instances)} & \x{inst} &::=&
  \{{\K{func}} \; \x{a}^\ast,\; {\K{global}} \; \x{a}^\ast,\; {\K{table}} \; \x{a}^?,\; {\K{mem}} \; \x{a}^?\} \\
\text{(function closures)} & \x{cl} &::=&
  \{{\K{instance\_ind}} \; \x{a},\; {\K{code}} \; \x{func}\} ~|~
  \{{\K{host}} \; ...\} \\
  %\hfill \quad \text{(where $\x{func}$ is not an import and has all exports $\x{ex}^\ast$ erased)} \\
\text{(table instances)} & \x{ti} &::=&
  (\x{a}^?)^\ast \\
%  \{{\K{data}} = \x{fi}^\ast,\; {\K{max}} = n^?\} \\
\text{(memory instances)} & \x{mi} &::=&
  \x{byte}^\ast \\%
\text{(store)} & s &::=&
  \{{\K{inst}} \; \x{inst}^\ast,\; {\K{func}} \; \x{cl}^\ast,\; {\K{global}} \; (\K{mut}^?~\x{v})^\ast,\; {\K{table}} \; \x{ti}^\ast,\; {\K{mem} \; (\x{sec}, \x{mi})^\ast}\} \\[1ex]

\text{(administrative instructions)} & e &::=&
  \dots ~|~
  \KK{trap} ~|~
  \KK{call}~\x{cl} ~|~
  \KK{label}_n\!\{e^\ast\}~e^\ast~\KK{end} ~|~
  \KK{local}_n\!\{i; \x{v}^\ast\}~e^\ast~\KK{end}\\

\text{(local contexts)} & L^0 &::=&
  \x{v}^\ast~[\K\textunderscore]~e^\ast \\ %~|~ \\
 & L^{k+1} &::=&
  \x{v}^\ast~\KK{label}_n\!\{e^\ast\}~L^k~\KK{end}~e^\ast \\[1ex]

\text{(configurations)} & \x{c} &::=&
  \x{s}; \x{v}^\ast; \x{e}^\ast \\[1ex]
\end{array}
\end{array}
$$

$$
\fontsize{9pt}{9pt}
\begin{array}{@{}rcl@{}}
s; \x{vs};~(\K{s}N.\KK{const}~c)~t_2\KK{.declassify}~t_1&\evalto_i&
  s; \x{vs};~(\K{i}N.\KK{const}~c) \\
s; \x{vs};~(\K{i}N.\KK{const}~c)~t_2\KK{.classify}~t_1&\evalto_i&
  s; \x{vs};~(\K{s}N.\KK{const}~c) \\
s; \x{vs};~\x{v}_1~\x{v}_2~((\KK{i32}~\x{sec})\KK{.const}~0)~\KK{select}~\x{sec}' &\evalto_i&
 s; \x{vs}; \x{v}_2 \\
s; \x{vs};~\x{v}_1~\x{v}_2~((\KK{i32}~\x{sec})\KK{.const}~k+1)~\KK{select}~\x{sec}' &\evalto_i&
  s; \x{vs};\x{v}_1 \\
[1ex]
\end{array}
$$

%\vspace{-1\baselineskip}

\caption{Selected \ctwasm semantic definitions,  extended from~\cite{Haas:2017:BWU:3062341.3062363}}
\label{fig:reduction}

\end{figure*}


==> figures/function_typing.tex <==
\begin{figure}

\begin{displaymath}
\prftree[r]{invoke reduction}
{
\text{\textbf{cl} = \textbf{func\_native} i (\textit{tr, $(t1s \rightarrow t2s)$}) ts es}\hspace{0.5cm}
}
{
\text{length vs = length t1s}
}
{
\text{vs; (\textbf{invoke cl})} \leadsto \text{\textbf{local} n i (vs; zeros(ts)) [\textbf{block} $([] \rightarrow t2s)$ es]}
}
\end{displaymath}

\begin{displaymath}
\prftree[r]{invoke typing}
{
\pbox{0.75\textwidth}{
\centering
\pbox{0.6\textwidth}{$
\mathcal{C}_\mathcal{S} = (\text{insts }\mathcal{S})\text{!i}\text{, trust := \textit{tr}, locals := } ... \text{, labels := } ... \text{, return := } ...
$}
\pbox{0.6\textwidth}{
\textbf{cl} = \textbf{func\_native} i (\textit{tr, tf}) ts es \hspace{0.5cm}
}
\pbox{0.6\textwidth}{$
\mathcal{S}\ \mathcal{C}_\mathcal{S} \vdash \text{es} : \textit{tf} \hspace{0.5cm}
$}
\pbox{0.6\textwidth}{$
\text{trust }\mathcal{C} \succ_{\text{tr}} tr
$}
}
}
{
\mathcal{S}\ \mathcal{C} \vdash [\textbf{invoke cl}] : \textit{tf}
}
\end{displaymath}

\begin{displaymath}
\prftree[r]{local typing}
{
\pbox{0.5\textwidth}{
\centering
\pbox{0.5\textwidth}{$
\mathcal{C}_\mathcal{S} = (\text{insts }\mathcal{S})\text{!i}\text{, trust := } (\text{trust }\mathcal{C})\text{, locals := } ... \text{, return := } ...
$}
\pbox{0.5\textwidth}{$
\mathcal{S}\ \mathcal{C}_\mathcal{S} \vdash \text{es} : [] \rightarrow ts
$}
}
}
{
\mathcal{S}\ \mathcal{C} \vdash [\text{\textbf{local} n i vs es}] : [] \rightarrow ts
}
\end{displaymath}

 \caption{Intermediate reductions of function calls and their (abbreviated) typing rules.}
\label{fig:function_typing}
\end{figure}

